DocLLM: A layout-aware generative language model for multimodal document understanding

Enterprise documents such as forms, invoices, receipts, reports, contracts, and other similar records, often carry rich semantics at the intersection of textual and spatial modalities. The visual cues offered by their complex layouts play a crucial role in comprehending these documents effectively. In this paper, we present DocLLM, a lightweight extension to traditional large language models (LLMs) for reasoning over visual documents, taking into account both textual semantics and spatial layout. Our model differs from existing multimodal LLMs by avoiding expensive image encoders and focuses exclusively on bounding box information to incorporate the spatial layout structure. Specifically, the cross-alignment between text and spatial modalities is captured by decomposing the attention mechanism in classical transformers to a set of disentangled matrices. Furthermore, we devise a pre-training objective that learns to infill text segments. This approach allows us to address irregular layouts and heterogeneous content frequently encountered in visual documents. The pre-trained model is fine-tuned using a large-scale instruction dataset, covering four core document intelligence tasks. We demonstrate that our solution outperforms SotA LLMs on 14 out of 16 datasets across all tasks, and generalizes well to 4 out of 5 previously unseen datasets.

==> sec_TODO.tex <==
\begin{itemize}
  \item adding appendices 
  \item \textbf{adding visual/qualitative examples}/overview of error modes
  \item splitting the causal-decoder and prefix-decoder attention illustration to two figures and using subfigures to insert. 
  \item updating the legend of Figure 4, Performance comparison between causal decoder and prefix decoder
  \item (for the ACL submission): moving Figure 1 to the cover page
  \item adding QLoRA fine tuning experiments with Llama2-7B OCR
  \item breaking the instruction-tuning part into two (dataset details to move to the expts section)
  \item benchmarking against GPT-4V
\end{itemize}

==> sec_appendices.tex <==
\appendix
\section{Prompting}
the template we used is as follows:


f"""Based on the given Document, {question}

Please provide only the answer (no decorations or explanations). Extract from the document when possible.

Use the following format to answer:
Answer:<answer>

Document:```{doc}```
"""

\section{Other training details}
We employed 8 AWS-based A10g GPUs, each equipped with 24GB of memory, for the pre-training process. The pre-training model is configured to run for a maximum of 5 epochs. Details of the model layer split are in Table \ref{tb:gpu_split_situ}, and GPU memory usage are provided in Table \ref{gpu_processes}.

\begin{table}[]
\centering
\caption{\label{tb:gpu_split_situ}7B model split situation}
\begin{tabular}{|c|c|}
\hline
GPU & Modules \\
\hline
0 & model.embed\_tokens, model.spatial\_embeddings, model.position\_embeddings \\
1 & Layer 0, Layer 1, Layer 2, Layer 3 \\
2 & Layer 4, Layer 5, Layer 6, Layer 7 \\
3 & Layer 8, Layer 9, Layer 10, Layer 11, Layer 12 \\
4 & Layer 13, Layer 14, Layer 15, Layer 16, Layer 17 \\
5 & Layer 18, Layer 19, Layer 20, Layer 21, Layer 22 \\
6 & Layer 23, Layer 24, Layer 25, Layer 26, Layer 27 \\
7 & Layer 28, Layer 29, Layer 30, Layer 31, norm, lm\_head \\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
    \centering
    \caption{\label{tab:gpu_processes}GPU Processes Information}
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \textbf{GPU} & \textbf{GI} & \textbf{CI} & \textbf{PID} & \textbf{Type} & \textbf{Process name} & \textbf{GPU Memory Usage} \\
        \hline
        0 & N/A & N/A & 72863 & C & python & 5250MiB \\
        1 & N/A & N/A & 72863 & C & python & 14358MiB \\
        2 & N/A & N/A & 72863 & C & python & 21740MiB \\
        3 & N/A & N/A & 72863 & C & python & 21740MiB \\
        4 & N/A & N/A & 72863 & C & python & 21740MiB \\
        5 & N/A & N/A & 72863 & C & python & 21740MiB \\
        6 & N/A & N/A & 72863 & C & python & 21740MiB \\
        7 & N/A & N/A & 72863 & C & python & 20136MiB \\
        \hline
    \end{tabular}
\end{table}

